Collaborative Control for Geometry-Conditioned PBR Image Generation

Graphics pipelines require physically-based rendering (PBR) materials, yet current 3D content generation approaches are built on RGB models. We propose to model the PBR image distribution directly, avoiding photometric inaccuracies in RGB generation and the inherent ambiguity in extracting PBR from RGB. As existing paradigms for cross-modal fine-tuning are not suited for PBR generation due to both a lack of data and the high dimensionality of the output modalities, we propose to train a new PBR model that is tightly linked to a frozen RGB model using a novel cross-network communication paradigm. As the base RGB model is fully frozen, the proposed method retains its general performance and remains compatible with e.g. IPAdapters for that base model.

==> img/tikz/control_diagram_parts/animate_anyone.tex <==
\begin{tikzpicture}[
    node distance=0.2cm, 
    font={\fontsize{8pt}{10}\selectfont},
    layer/.style={draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.2cm, rounded corners=1pt},
    textlayer/.style={draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.1cm, rounded corners=1pt},
    encoder/.style={trapezium, trapezium angle=60, text width=0.3cm, text height=0.4cm, shape border rotate=0, draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.1cm, rounded corners=1pt},
    decoder/.style={trapezium, trapezium angle=60, text width=0.3cm, text height=0.4cm, shape border rotate=180, draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.1cm, rounded corners=1pt},
    label/.style={font=\scriptsize, text width=1.2cm, align=center}
]

\node[encoder={blueish}] (enc) {};
\node[decoder={blueish}, above=-0.5pt of enc] (dec) {};
 
\node[encoder={orange}, right=0.5cm of enc] (control_enc) {};
\node[decoder={orange}, above=-0.5pt of control_enc] (control_dec) {};

\coordinate[below=of enc] (enc_in);
\coordinate[below=of control_enc] (control_enc_in);
\coordinate[above=of dec] (dec_out);
\coordinate[above=of control_dec] (control_dec_out);

\draw[-stealth, draw=dark_green] (enc_in) -- (enc);
\draw[-stealth, draw=dark_green] (control_enc_in) -- (control_enc);
\draw[-stealth, draw=dark_green] (control_dec) -- (control_dec_out);
\draw[-stealth, draw=orange, thick] (enc) -- (control_enc);
\draw[-stealth, draw=orange, thick] (dec) -- (control_dec);
\end{tikzpicture}


==> img/tikz/control_diagram_parts/collaborative_control.tex <==
\begin{tikzpicture}[
    node distance=0.2cm, 
    font={\fontsize{8pt}{10}\selectfont},
    layer/.style={draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.2cm, rounded corners=1pt},
    textlayer/.style={draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.1cm, rounded corners=1pt},
    encoder/.style={trapezium, trapezium angle=60, text width=0.3cm, text height=0.4cm, shape border rotate=0, draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.1cm, rounded corners=1pt},
    decoder/.style={trapezium, trapezium angle=60, text width=0.3cm, text height=0.4cm, shape border rotate=180, draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.1cm, rounded corners=1pt},
    label/.style={font=\scriptsize, text width=1.2cm, align=center}
]

\node[encoder={blueish}] (enc) {};
\node[decoder={blueish}, above=-0.5pt of enc] (dec) {};
 
\node[encoder={orange}, right=0.5cm of enc] (control_enc) {};
\node[decoder={orange}, above=-0.5pt of control_enc] (control_dec) {};

\coordinate[below=of enc] (enc_in);
\coordinate[below=of control_enc] (control_enc_in);
\coordinate[above=of dec] (dec_out);
\coordinate[above=of control_dec] (control_dec_out);

\draw[-stealth, draw=dark_green] (enc_in) -- (enc);
\draw[-stealth, draw=dark_green] (control_enc_in) -- (control_enc);
\draw[-stealth, draw=dark_green] (dec) -- (dec_out);
\draw[-stealth, draw=dark_green] (control_dec) -- (control_dec_out);
\draw[stealth-stealth, draw=orange, thick] (enc) -- (control_enc);
\draw[stealth-stealth, draw=orange, thick] (dec) -- (control_dec);
\end{tikzpicture}


==> img/tikz/control_diagram_parts/control_net.tex <==
\begin{tikzpicture}[
    node distance=0.2cm, 
    font={\fontsize{8pt}{10}\selectfont},
    layer/.style={draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.2cm, rounded corners=1pt},
    textlayer/.style={draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.1cm, rounded corners=1pt},
    encoder/.style={trapezium, trapezium angle=60, text width=0.3cm, text height=0.4cm, shape border rotate=0, draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.1cm, rounded corners=1pt},
    decoder/.style={trapezium, trapezium angle=60, text width=0.3cm, text height=0.4cm, shape border rotate=180, draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.1cm, rounded corners=1pt},
    label/.style={font=\scriptsize, text width=1.2cm, align=center}
]

\node[encoder={blueish}] (enc) {};
\node[decoder={blueish}, above=-0.5pt of enc] (dec) {};
 
\node[encoder={orange}, right=0.5cm of enc] (control_enc) {};

\coordinate[below=of enc] (enc_in);
\coordinate[below=of control_enc] (control_enc_in);
\coordinate[above=of dec] (dec_out);

\draw[-stealth, draw=dark_green] (enc_in) -- (enc);
\draw[-stealth, draw=dark_green] (control_enc_in) -- (control_enc);
\draw[-stealth, draw=dark_green] (dec) -- (dec_out);
\draw[-stealth, draw=orange, thick] (control_enc) |- (dec);
\end{tikzpicture}


==> img/tikz/control_diagram_parts/control_net_xs.tex <==
\begin{tikzpicture}[
    node distance=0.2cm, 
    font={\fontsize{8pt}{10}\selectfont},
    layer/.style={draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.2cm, rounded corners=1pt},
    textlayer/.style={draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.1cm, rounded corners=1pt},
    encoder/.style={trapezium, trapezium angle=60, text width=0.3cm, text height=0.4cm, shape border rotate=0, draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.1cm, rounded corners=1pt},
    decoder/.style={trapezium, trapezium angle=60, text width=0.3cm, text height=0.4cm, shape border rotate=180, draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.1cm, rounded corners=1pt},
    label/.style={font=\scriptsize, text width=1.2cm, align=center}
]

\node[encoder={blueish}] (enc) {};
\node[decoder={blueish}, above=-0.5pt of enc] (dec) {};
 
\node[encoder={orange}, right=0.5cm of enc] (control_enc) {};

\coordinate[below=of enc] (enc_in);
\coordinate[below=of control_enc] (control_enc_in);
\coordinate[above=of dec] (dec_out);

\draw[-stealth, draw=dark_green] (enc_in) -- (enc);
\draw[-stealth, draw=dark_green] (control_enc_in) -- (control_enc);
\draw[-stealth, draw=dark_green] (dec) -- (dec_out);
\draw[-stealth, draw=orange, thick] (control_enc) |- (dec);
\draw[-stealth, draw=orange, thick] (control_enc) -- (enc);
\end{tikzpicture}


==> img/tikz/overview_parts/collaborative_control_comm.tex <==
\begin{tikzpicture}[
    node distance=0.5cm, 
    font={\fontsize{8pt}{10}\selectfont},
    layer/.style={draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.2cm, rounded corners=1pt},
    textlayer/.style={draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.1cm, rounded corners=1pt},
    encoder/.style={isosceles triangle,isosceles triangle apex angle=60,shape border rotate=0,anchor=apex,draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.1cm, rounded corners=1pt},
    decoder/.style={isosceles triangle,isosceles triangle apex angle=60,shape border rotate=180,anchor=apex,draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.1cm, rounded corners=1pt},
    label/.style={font=\scriptsize, text width=1.2cm, align=center}
]


\node[draw=blueish, fill=white, text width=1cm, text height=0.1cm, rounded corners=1pt, line width=0.5pt, font=\tiny] (rgb_cross_attn) at (0, 0) {Cross Attention};
\node[draw=blueish, fill=white, text width=1cm, text height=0.1cm, rounded corners=1pt, line width=0.5pt, font=\tiny, below=0.75cm of rgb_cross_attn] (rgb_self_attn) {Self\phantom{as} Attention};
\node[draw=blueish, fill=white, text width=1cm, text height=0.1cm, rounded corners=1pt, line width=0.5pt, font=\tiny, below=0.2cm of rgb_self_attn] (rgb_conv) {Conv Block};

\begin{scope}[on background layer]
    \draw[layer={blueish}, rounded corners=1pt,line width=1.5pt] ($(rgb_cross_attn.north west)+(-0.075,0.075)$)  rectangle ($(rgb_conv.south east)+(0.075,-0.075)$);
\end{scope}

\node[right=of rgb_cross_attn, font=\tiny, draw=dark_green, fill=white, rounded rectangle, rounded rectangle east arc=0pt, line width=1pt] (cross_attn_rgb) {RGB};
\node[right=0cm of cross_attn_rgb, font=\tiny, draw=dark_green, fill=white, rounded rectangle, rounded rectangle west arc=0pt, line width=1pt] (cross_attn_pbr) {PBR};
\coordinate (cross_attn_comm_rgb_pbr) at ($(cross_attn_pbr)!0.5!(cross_attn_rgb)$);

\node[right=of rgb_self_attn, font=\tiny, draw=dark_green, fill=white, rounded rectangle, rounded rectangle east arc=0pt, line width=1pt] (self_attn_rgb) {RGB};
\node[right=0cm of self_attn_rgb, font=\tiny, draw=dark_green, fill=white, rounded rectangle, rounded rectangle west arc=0pt, line width=1pt] (self_attn_pbr) {PBR};
\coordinate (self_attn_comm_rgb_pbr) at ($(self_attn_pbr)!0.5!(self_attn_rgb)$);

\node[textlayer={orange}, font=\tiny, align=center, text width=1.75cm, inner sep=0.05cm] (cross_comm) at ($(cross_attn_comm_rgb_pbr)!0.5!(self_attn_comm_rgb_pbr)$) {Cross-Network Communication};

\node[draw=orange, fill=white, text width=1cm, text height=0.1cm, rounded corners=1pt, line width=0.5pt, font=\tiny, right=of self_attn_pbr] (pbr_self_attention) {Self\phantom{as} Attention};
\node[draw=orange, fill=white, text width=1cm, text height=0.1cm, rounded corners=1pt, line width=0.5pt, font=\tiny, below=0.2cm of pbr_self_attention] (pbr_conv) {Conv Block};

\coordinate (pbr_out_point) at (cross_attn_pbr-|pbr_self_attention);
\begin{scope}[on background layer]
    \draw[layer={orange}, rounded corners=1pt,line width=1.5pt] ($(pbr_self_attention.west|-rgb_cross_attn.north)+(-0.075,0.075)$)  rectangle ($(pbr_conv.south east)+(0.075,-0.075)$);
\end{scope}

\draw[-stealth, draw=dark_green] (rgb_conv) -- (rgb_self_attn);
\draw[-stealth, draw=dark_green] (pbr_conv) -- (pbr_self_attention);
\draw[-stealth, draw=dark_green, shorten <=0.15cm] (self_attn_comm_rgb_pbr) -- (cross_comm);
\draw[-stealth, draw=dark_green, shorten >=0.15cm] (cross_comm) -- (cross_attn_comm_rgb_pbr);
\draw[-stealth, draw=dark_green, shorten >=0.075cm] (cross_attn_rgb) -- (rgb_cross_attn);
\draw[draw=dark_green] (cross_attn_pbr) -- (pbr_out_point);

\coordinate[left=of rgb_cross_attn] (text_input);
\coordinate[above=of rgb_cross_attn] (rgb_output);
\coordinate (pbr_output) at (rgb_output-|pbr_out_point);

\coordinate[below=of rgb_conv] (rgb_input);
\coordinate[below=of pbr_conv] (pbr_input);

\draw[-stealth, draw=purple, shorten >=0.075cm] (text_input) -- (rgb_cross_attn);
\draw[-stealth, draw=dark_green, shorten <=0.075cm] (rgb_cross_attn) -- (rgb_output);
\draw[-stealth, draw=dark_green] (pbr_out_point) -- (pbr_output);

\draw[-stealth, draw=dark_green, shorten >=0.075cm] (rgb_input) -- (rgb_conv);
\draw[-stealth, draw=dark_green, shorten >=0.075cm] (pbr_input) -- (pbr_conv);

\draw[-stealth, draw=dark_green, shorten <=0.075cm] (rgb_self_attn) -- (self_attn_rgb);
\draw[-stealth, draw=dark_green, shorten <=0.075cm] (pbr_self_attention) -- (self_attn_pbr);

\node[font=\tiny, text width=1cm, align=center] at (cross_comm-|rgb_self_attn) {RGB Block};
\node[font=\tiny, text width=1cm, align=center] at (cross_comm-|pbr_self_attention) {PBR Block};

\end{tikzpicture}


==> img/tikz/overview_parts/collaborative_control_main.tex <==
\begin{tikzpicture}[
    node distance=0.5cm, 
    font={\fontsize{8pt}{10}\selectfont},
    layer/.style={draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.2cm, rounded corners=1pt},
    textlayer/.style={draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.1cm, rounded corners=1pt},
    encoder/.style={isosceles triangle,isosceles triangle apex angle=60,shape border rotate=0,anchor=apex,draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.1cm, rounded corners=1pt},
    decoder/.style={isosceles triangle,isosceles triangle apex angle=60,shape border rotate=180,anchor=apex,draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.1cm, rounded corners=1pt},
    label/.style={font=\scriptsize, text width=1.2cm, align=center}
]

\begin{scope}[shift={(0,0)}]
\node[draw=blueish, fill=white, text width=1.25cm, text height=0.1cm, rounded corners=1pt, line width=0.5pt] (rgb_unet-1) at (0, 0) {};
\node[draw=blueish, fill=white, text width=0.7cm, text height=0.1cm, below=0.1cm of rgb_unet-1, rounded corners=1pt, line width=0.5pt] (rgb_unet-2) {};
\node[draw=blueish, fill=white, text width=0.25cm, text height=0.1cm, below=0.1cm of rgb_unet-2, rounded corners=1pt, line width=0.5pt] (rgb_unet-3) {};
\node[draw=blueish, fill=white, text width=0.25cm, text height=0.1cm, below=0.1cm of rgb_unet-3, rounded corners=1pt, line width=0.5pt] (rgb_unet-4) {};
\node[draw=blueish, fill=white, text width=0.7cm, text height=0.1cm, below=0.1cm of rgb_unet-4, rounded corners=1pt, line width=0.5pt] (rgb_unet-5) {};
\node[draw=blueish, fill=white, text width=1.25cm, text height=0.1cm, below=0.1cm of rgb_unet-5, rounded corners=1pt, line width=0.5pt] (rgb_unet-6) {};

\begin{scope}[on background layer]
    \draw[fill=blueish!20, draw=blueish, rounded corners=1pt,line width=1.5pt] 
        ($(rgb_unet-1.north west)+(-0.275,0.15)$) -- 
        ($(rgb_unet-3.west)!0.5!(rgb_unet-4.west)+(-0.275,0)$) -- 
        ($(rgb_unet-6.south west)+(-0.275,-0.15)$) -- 
        ($(rgb_unet-6.south east)+(0.275,-0.15)$) -- 
        ($(rgb_unet-3.east)!0.5!(rgb_unet-4.east)+(0.275,0)$) -- 
        ($(rgb_unet-1.north east)+(0.275,0.15)$) -- cycle;%
\end{scope}
\end{scope}

\begin{scope}[shift={(2.9,0)}]
    \node[draw=orange, fill=white, text width=1.25cm, text height=0.1cm, rounded corners=1pt, line width=0.5pt] (pbr_unet-1) at (0, 0) {};
    \node[draw=orange, fill=white, text width=0.7cm, text height=0.1cm, below=0.1cm of pbr_unet-1, rounded corners=1pt, line width=0.5pt] (pbr_unet-2) {};
    \node[draw=orange, fill=white, text width=0.25cm, text height=0.1cm, below=0.1cm of pbr_unet-2, rounded corners=1pt, line width=0.5pt] (pbr_unet-3) {};
    \node[draw=orange, fill=white, text width=0.25cm, text height=0.1cm, below=0.1cm of pbr_unet-3, rounded corners=1pt, line width=0.5pt] (pbr_unet-4) {};
    \node[draw=orange, fill=white, text width=0.7cm, text height=0.1cm, below=0.1cm of pbr_unet-4, rounded corners=1pt, line width=0.5pt] (pbr_unet-5) {};
    \node[draw=orange, fill=white, text width=1.25cm, text height=0.1cm, below=0.1cm of pbr_unet-5, rounded corners=1pt, line width=0.5pt] (pbr_unet-6) {};
    
    \begin{scope}[on background layer]
        \draw[fill=orange!20, draw=orange, rounded corners=1pt, line width=1.5pt] 
            ($(pbr_unet-1.north west)+(-0.275,0.15)$) -- 
            ($(pbr_unet-3.west)!0.5!(pbr_unet-4.west)+(-0.275,0)$) -- 
            ($(pbr_unet-6.south west)+(-0.275,-0.15)$) -- 
            ($(pbr_unet-6.south east)+(0.275,-0.15)$) -- 
            ($(pbr_unet-3.east)!0.5!(pbr_unet-4.east)+(0.275,0)$) -- 
            ($(pbr_unet-1.north east)+(0.275,0.15)$) -- cycle;%
    \end{scope}
\end{scope}

\foreach \i in {1,2,...,6} {
    \node[draw=orange, fill=orange!20, text width=0.4cm, text height=0.01cm, rounded corners=1pt, line width=0.5pt] (translate-\i) at ($(rgb_unet-\i)!0.5!(pbr_unet-\i)$) {};
};

\node[left=0.6cm of $(rgb_unet-1.west)!0.5!(rgb_unet-6.west)$, font=\tiny] {\rotatebox{90}{\faSnowflake[regular] \! Frozen RGB Diffusion}};
\node[right=0.3cm of $(pbr_unet-1.east)!0.5!(pbr_unet-6.east)$, font=\tiny] {\rotatebox{90}{\faBookOpen \, Trained PBR Diffusion}};


\node[textlayer={dark_green}, below=of rgb_unet-6, align=center, text width=0.8cm, font=\tiny] (noisy_rgb_label) {Noisy RGB};
\node[textlayer={purple}, left=0.2cm of noisy_rgb_label, align=center, text width=0.8cm, font=\tiny] (text_prompt) {Text prompt};

\draw [-stealth] (noisy_rgb_label) -- (rgb_unet-6);

\coordinate (below_pbr) at (noisy_rgb_label-|pbr_unet-6);
\node[textlayer={dark_green}, left=0.1cm of below_pbr, align=center, text width=0.8cm, font=\tiny] (noisy_pbr) {Noisy PBR};
\node[textlayer={dark_green}, right=0.1cm of below_pbr, align=center, text width=1.2cm, font=\tiny] (geometry_conditioning) {Geometry Condition};

\draw [-stealth] (noisy_pbr) -- (pbr_unet-6);
\draw [-stealth] (geometry_conditioning) -- (pbr_unet-6);

\foreach \i in {1,2,...,6} {
    \draw [-stealth] (text_prompt) |- (rgb_unet-\i);
    \draw [stealth-stealth] (rgb_unet-\i) -- (translate-\i);
    \draw [stealth-stealth] (pbr_unet-\i) -- (translate-\i);
};

\node[textlayer={dark_green}, above=of rgb_unet-1, align=center, text width=0.95cm, font=\tiny] (denoised_rgb_label) {Denoised RGB};
\node[textlayer={dark_green}, above=of pbr_unet-1, align=center, text width=0.95cm, font=\tiny] (denoised_pbr_label) {Denoised PBR};

\draw[-stealth] (rgb_unet-1) -- (denoised_rgb_label);
\draw[-stealth] (pbr_unet-1) -- (denoised_pbr_label);


\end{tikzpicture}

